Arabic Multi-Dialect Segmentation: bi-LSTM-CRF vs. SVM

Arabic word segmentation is essential for a variety of NLP applications such as machine translation and information retrieval. Segmentation entails breaking words into their constituent stems, affixes and clitics. In this paper, we compare two approaches for segmenting four major Arabic dialects using only several thousand training examples for each dialect. The two approaches involve posing the problem as a ranking problem, where an SVM ranker picks the best segmentation, and as a sequence labeling problem, where a bi-LSTM RNN coupled with CRF determines where best to segment words. We are able to achieve solid segmentation results for all dialects using rather limited training data. We also show that employing Modern Standard Arabic data for domain adaptation and assuming context independence improve overall results.

==> 04_dataset.tex <==
% % \textcolor{red}{(Hamdy)}
% We used the dataset described in \cite{darwish2014verifiably} which they tested in dialect identification task to distinguish between dialectal Egyptian and MSA. It contains 350 tweets with more than 8,000 words including 3,000 unique words written in Egyptian dialect. The tweets have much dialectal content covering most of dialectal Egyptian phonological, morphological, and syntactic phenomena. It also contains Twitter-specific aspects of the text, such as \#hashtags, $@$mentions, emoticons and URLs.

% We manually annotated each word in this corpus to provide: CODA-compliant writing \cite{habash2012conventional}, segmentation, stem, lemma, and POS, also the corresponding MSA word, MSA segmentation, and MSA POS. We share the dataset\footnote{Dataset is available at www.hidden-for-blind-review.com} to reproduce test results and help in other tasks such as CODA'fication of dialectal text, dialectal POS tagging and dialect to MSA conversion. Table~\ref{annotations} shows an annotation example of the word \<بيقولك> ``byqwlk'' (he is saying to you).

% \begin{table}[h]
% \begin{center}
% \begin{tabular}{|l|l|}
% \hline \bf Field & \bf Annotation \\ \hline
% Orig. word & \<بيقولك> ``byqwlk''\\
% (Glossary) & he is saying to you \\
% Orig. Segm. & \<ك>+\<ل>+\<يقو>+\<ب>``b+yqw+l+k''\\
% CODA & \<بيقول لك> ``byqwl lk''\\
% CODA Segm. & \<ك>+\<يقول ل>+\<ب>``b+yqwl l+k''\\
% POS & PROG\_PART+V PREP+PRON\\
% Stem & \<يقول ل> ``yqwl l''\\ 
% lemma & \<قال ل> ``qAl l''\\ 
% MSA & \<يقول لك> ``yqwl lk''\\
% MSA Segm. & \<ك>+\<يقول ل>``yqwl l+k''\\
% MSA POS & V PREP+PRON\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Annotation Example}
% \label{annotations}
% \end{table}

% \begin{table}
% \begin{center}
% \begin{tabular}{c|c|c}
% Dialect & No of Tweets & No of Tokens \\ \hline
% Egyptian & 356 & 6,721 \\
% Levantine & 350 &  6,648 \\
% Gulf & 385 & 6,844 \\
% Maghrebi & 349 & 5,495 \\ \hline
% \end{tabular}
% \end{center}
% \end{table}
% \textcolor{red}{Hamdy: We have exactly 350 tweets in all dialects. Right? Does "No of Tokens" contain also punct, numbers, URL's, etc.?}
